XtremeDistil: Multi-stage Distillation for Massive Multilingual Models

Deep and large pre-trained language models are the state-of-the-art for various natural language processing tasks. However, the huge size of these models could be a deterrent to use them in practice. Some recent and concurrent works use knowledge distillation to compress these huge models into shallow ones. In this work we study knowledge distillation with a focus on multi-lingual Named Entity Recognition (NER). In particular, we study several distillation strategies and propose a stage-wise optimization scheme leveraging teacher internal representations that is agnostic of teacher architecture and show that it outperforms strategies employed in prior works. Additionally, we investigate the role of several factors like the amount of unlabeled data, annotation resources, model architecture and inference latency to name a few. We show that our approach leads to massive compression of MBERT-like teacher models by upto 35x in terms of parameters and 51x in terms of latency for batch inference while retaining 95% of its F1-score for NER over 41 languages.

==> experiments-old.tex <==
\section{Experiments}

\subsubsection{Dataset Description}
We perform large-scale experiments with data from four domains for different tasks as summarized in Table~\ref{tab:dataset}. Two of these datasets IMDB~\citep{DBLP:conf/acl/MaasDPHNP11} and Elec~\citep{DBLP:conf/recsys/McAuleyL13} are used for sentiment classification for movie reviews and Amazon electronics product reviews respectively. The other two datasets DbPedia~\citep{DBLP:conf/nips/ZhangZL15} and Ag News~\citep{DBLP:conf/nips/ZhangZL15} are used for topic classification of Wikipedia and news articles respectively. These datasets have been extensively used for benchmarking in several other text classification tasks~\citep{DBLP:conf/nips/ZhangZL15,DBLP:journals/corr/Johnson014,DBLP:conf/iclr/MiyatoDG17}

\begin{table}[]
    \centering
    \begin{tabular}{lccccc}
        \toprule
         { Dataset} & { Class} & { Train} & { Test} & { Unlabeled} & { \#W}\\\midrule
         IMDB & 2 & 25K & 25K & 50K & 235\\
         DBPedia & 14 & 560K & 70K & - & 51\\
         AG News & 4 & 120K & 7.6K & - & 40\\
         Elec & 2 & 25K & 25K & 200K & 108\\
         %Yelp & Rating & 5 & 650K & 50K & - & 135\\
         \bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Full dataset summary (W: average words per doc).}
    %\vspace{-1em}
    \label{tab:dataset}
\end{table}

\subsubsection{Evaluation Questions} In the experiments we want to answer the following questions:

\begin{itemize}
    \item How much can we improve the performance of student models by distillation?
    \item Does distillation improve with a better teacher?
    \item What is the impact of soft vs. hard distillation for pre-trained language models?
    \item When does distillation provide the maximum value?
    %\item What is the impact of the number of labeled instances on distillation?
    %\item How much uncertainty of the deep pre-trained language models can we explore via the distillation process?
\end{itemize}

\subsubsection{Parameter Configurations}

We split each labeled dataset into $90\%$ for training and $10\%$ for validation and report aggregate results on the blind test set based on the validation set. We implement our framework in Tensorflow and use four Tesla V100 gpus for experimentation. We use Adadelta~\citep{DBLP:journals/corr/abs-1212-5701} as the optimization algorithm with early stopping and use the best model found so far from the validation loss. Adadelta does not require an initial learning rate. We also experimented with Adam~\citep{DBLP:journals/corr/KingmaB14}. We found it to converge faster but the results were often sub-optimal compared to Adadelta in our setting. %Similar observations have been reported in~\citep{DBLP:journals/corr/WuSCLNMKCGMKSJL16}. 
To regularize our network, we used dropouts ($rate=0.4$) after every layer as well as recurrent dropouts ($rate=0.2$) in the BiLSTM. We use pre-trained $300$ dimensional word embeddings from Glove~\citep{DBLP:conf/emnlp/PenningtonSM14} to initialize our model that are fine-tuned during training. Words not present in the vocabulary are randomly initialized with $\mathcal{U}(-.1, .1)$. We set the number of hidden units in the LSTM to $600$ for each direction ($1200$ for BiLSTM), batch size to 64, and $\alpha=\beta=10, \gamma=1$.
%Table~\ref{tab:hyper} shows the model hyper-parameters.

\begin{comment}
\begin{table}[]
    \centering
    \begin{tabular}{l|c}
    \toprule
         Word embedding dimension & 300\\
         BiLSTM hidden units & $2 \times 600$  \\
         Batch size & 64 \\
         $\alpha, \beta$ & 10\\
         $\gamma$ & 1\\
         Layer dropout rate & 0.4\\
         Recurrent dropout rate & 0.2\\\midrule
    \end{tabular}
    \begin{tabular}{c}
    Sequence length: 256 (Imdb), 128 (Elec), 90 (Dbpedia)\\ 
    80 (Ag News)%, 180 (Yelp)\\
    \\\bottomrule
    \end{tabular}
    \caption{Hyper-parameter configuration.}
    \label{tab:hyper}
\end{table}
\end{comment}

\subsubsection{Teacher Model}

We consider the state-of-the-art pre-trained language model BERT~\citep{DBLP:conf/naacl/DevlinCLT19} to be the teacher in our setting. Note that we do not make any assumptions about the architecture of the teacher; it is possible to plug-in any large pre-trained model in our framework.

BERT's model architecture is a multi-layer bidirectional Transformer encoder. We experiment with two configurations: (i) BERT Base consisting of 12 layers, 12 self-attention heads, and 768 dimensional hidden state representation with an overall 110 million parameters. (ii) BERT-Large consisting of 24 layers, 16 self-attention heads, and 1024 dimensional hidden state representation with an overall 340 million parameters. Pre-trained BERT Large models have two variants corresponding to different masking technique for pre-training. We use uncased, whole word masking models that are shown to be better than previous versions.

\subsubsection{Student Model}

We compare the following models:

\noindent (i) {\bf RNN Encoder} We consider BiLSTM encoders with word embeddings. The last hidden state of BiLSTM is fed into softmax for classification and the network parameters are trained by optimizing cross-entropy loss over labeled data as in Equations~\ref{eq:1} and~\ref{eq:2}. We use a basic tokenizer with this model that lowercases all words and splits by whitespace.

\noindent (ii) {\bf Student Model without Distillation} This extends the previous one with a max-pooling mechanism to consider all the BiLSTM hidden states instead of just the last one, while still generating a fixed length vector. Also, this and the subsequent models use wordpiece tokenization to normalize the input text. The student model is trained over labeled data using cross-entropy loss similar to the RNN encoder.

\noindent (iii) {\bf Student Model with Distillation} 
In this, we distil the aforementioned student with (soft / hard) targets and representations from the teacher. First, we fine-tune the teacher on labeled data and use it to generate the logits and hidden state representations for unlabeled instances. We train the student model end-to-end using cross-entropy loss on labeled instances (Equations~\ref{eq:1},~\ref{eq:2}) as well as logit loss (Equations~\ref{eq:3},~\ref{eq:4}) and representation loss (Equations~\ref{eq:5},~\ref{eq:6}) on the unlabeled data. We test three different learning strategies based on a joint optimization scheme as well as two stagewise ones with gradual unfreezing of the intermediate layers.

%Next, we discuss the first experimental setup with moderate number of training labels per class.

\subsection{Distillation with BERT Base}

In this setting, we consider BERT Base as the teacher with $110M$ parameters. For our setup, we require both labeled instances and unlabeled ones. However, some of the datasets like Dbpedia and AG News do not have any unlabeled instances. Therefore, we split all the labeled instances into two parts as follows: (a) randomly sample equal number of instances per class from the labeled data and use them for training as $D_L$. The total size of the training data for each task is made equal to the size of the test data. (b) all the remaining instances from the labeled data are stripped of labels and considered as unlabeled instances $D_U$ for our framework. Table~\ref{tab:moderate} shows the derived dataset statistics. Unless, otherwise mentioned all the experimental results in this paper are reported on this data split.

%** report the fully supervised results on the entire labeled dataset

\begin{table}[]
    \centering
    \begin{tabular}{lrrrr}
        \toprule
         { Dataset} & { Train} & { Test} & { Unlabeled} & { \#Train/Class} \\\midrule
         IMDB & 25K & 25K & 50K & 12.5K \\
         DBPedia & 70K & 70K & 490K & 5k\\
         AG News & 7.6K & 7.6K & 112.4K & 1.9K\\
         Elec & 25K & 25K & 200K & 12.5K\\
         %Yelp & 50K & 50K & 600K & 10K\\
         \bottomrule
    \end{tabular}
    %\vspace{-1em}
    \caption{Derived dataset summary.}
        %\vspace{-0.5em}
    \label{tab:moderate}
\end{table}

In this experiment, we compare the performance of the different student models with our distilled model. Table~\ref{tab:distil} summarizes the overall results. 

\begin{table}
    \centering
    \begin{tabular}{lcccc}
    \toprule
{ Dataset} & { RNN} & { Student} & { Student } & { BERT}\\
& & { no distil.} & { with distil.} & Base \\
\midrule
Ag News &	87.66 &	89.71 &	{\bf 92.33} &	92.12\\
IMDB &	89.93 &	89.37 &	91.22 &	{\bf 91.70}\\
Elec &	89.72 &	90.62 &	{\bf 93.55} &	{93.46}\\
Dbpedia	& 98.44	& 98.64	& 99.10	& {\bf 99.26}\\
%Yelp &  & 63.03 & {\bf 64.46} & 62.85\\
%\midrule
%\#Parameters & & & & 110M\\
\bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Distillation performance with BERT Base.}
    %\vspace{-1em}
    \label{tab:distil}
\end{table}

We observe that the student model with the max-pooling mechanism and wordpiece tokenization performs slightly better than the RNN encoder without these mechanisms. We observe that the RNN in general performs quite well in all the tasks for all of the datasets. With distillation we are further able to improve the student performance by $2$ percent on an average over all the tasks and match the teacher performance. From Table~\ref{tab:param} we observe that the distilled student model is $8.5x$ smaller in size than the teacher model in terms of the number of parameters. 

\begin{table}[h]
    \centering
    \begin{tabular}{lcccc}
    \toprule
{ Dataset} & { Distil with} & { Distil with} &  {\small BERT} & {\small	BERT}\\
 & { {\small BERT Base}} & { {\small BERT Large}} & {\small Base} & {\small Large} \\
\midrule
Ag News &	92.33 &	94.33 & 92.12	& {\bf 94.63}\\
IMDB &	91.22 &	91.70 &	91.70 &	{\bf 93.22}\\
Elec & 93.55 &	93.56 &	93.46 &	{\bf 94.27}\\
DbPedia	& 99.10	& 99.06 &	{\bf 99.26}	& 99.20\\
%Yelp &	64.46 &	& 62.85	& \\
\bottomrule
    \end{tabular}
    %\vspace{-1em}
    \caption{Better distillation with better teacher.}
%\vspace{-1em}
    \label{tab:teacher}
\end{table}


\subsection{Distillation with Larger and Better Teacher}

In this, we want to find out if the distillation performance improves with a more powerful teacher. We therefore experiment with BERT Large that is $3x$ larger than the Base version while  performing better in many of the tasks~\citep{DBLP:conf/naacl/DevlinCLT19}. Table~\ref{tab:teacher} shows the performance comparison. We observe that the student model performance improves marginally as the performance of the teacher improves. However, the gap in performance between the teacher and student also increases compared to the Base version indicating saturation in the the student network.

\subsubsection{Parameters} Table~\ref{tab:param} shows the number of parameters for the different models. Due to the usage of wordpiece tokenization with $30K$ fixed vocabulary size, all the model sizes have a fixed upper-bound irrespective of the dataset. We show the average number of parameters for the student model over different settings and configurations. Distilling the student with a larger teacher only increases the dimensionality of the transformation matrix $W^f$ to align the last hidden state representation of the teacher and student.

\begin{table}[h]
%\vspace{-0.5em}
    \centering
    \begin{tabular}{ccc}
    \toprule
    Distilled Student & BERT Base & BERT Large  \\\midrule
    13M & 110M & 340M\\\bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Parameters for the different models (M: millions).}
    %\vspace{-1em}
    \label{tab:param}
\end{table}

\subsection{Distilling Hard Targets vs. Soft Logits}

In the above experiments, we found the distillation performance with BERT Large to be better than that with BERT Base. Therefore, in this setting, we consider BERT Large as the teacher fine-tuned on labeled data. We use the fine-tuned teacher model to generate {\em hard predictions} on the {\em unlabeled data}. Thereafter, we train our student model jointly on the originally labeled data and BERT Large labeled instances.

Table~\ref{tab:hard} shows the distillation performance with hard targets versus leveraging the soft predictions and hidden state representations. We observe that the student model trained on hard BERT Large predictions perform extremely well. With soft distillation, we are able to further improve the performance across all the tasks.

\begin{table}[]
%\vspace{-1em}
    \centering
    \begin{tabular}{lcc}
    \toprule
    Dataset & Soft Distillation & Hard Distillation  \\
    \midrule
    AG News & {\bf 94.33} & 93.17\\ 
    Elec & {\bf 93.56} & 92.57 \\
    DBPedia & {\bf 99.06} & 98.97 \\
    IMDB & {\bf 91.70} & 91.21\\
    \bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Soft vs. hard distillation results with BERT Large.}
%\vspace{-1em}
    \label{tab:hard}
\end{table}

However, we observe the performance gap between soft distillation and hard targets from BERT to be narrow. To investigate this, we compute the variance in prediction probabilities of an instance from the teacher computed as follows. Consider $p_c(x_i)$ to be the probability of $x_i$ belonging to class $c$ as predicted by the teacher. Overall variance in prediction is given by $\sum_{i=1}^N Var(\langle p_1(x_i), p_2(x_i), \cdots p_c(x_i) \rangle) / N$ aggregated over all instances. Maximum variance is obtained when exactly one of these elements is one and rest are zeros.

Table~\ref{tab:variance} shows the prediction variance of the teacher for different tasks. The table also shows the maximum variance possible in case of one-hot predictions. We observe that BERT predictions are extremely confident almost similar to hard labels. The variance and therefore, the confidence further increases with the size of the teacher model. Since soft distillation relies on exploiting teacher uncertainties to improve the student -- such confident teacher makes this process extremely difficult. Nevertheless, we are still able to regularize the model with soft distillation and further improve the performance over that of hard targets from teacher.

\begin{table}[]
    \centering
    \begin{tabular}{lcccc}
    \toprule
Dataset &	BERT & BERT & Max. & Classes\\
 & Base & Large & Var. &\\
 \midrule
IMDB & 0.240 & 0.249 & 0.250 & 2 \\
Elec & 0.239 & 0.247 & 0.250 & 2\\
Ag News	& 0.173 & 0.185 & 0.188 & 4\\
Dbpedia &	0.066(0) &	0.066(1) & 0.066(3) & 14\\
\bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Variance in prediction probabilities of the teacher. Maximum variance is obtained when the teacher spits hard labels as opposed to soft predictions.}
    %\vspace{-0.5em}
    \label{tab:variance}
\end{table}

\subsection{ Distillation with Less Training Labels}

\subsubsection{$500$ labeled samples per class} In the previous experiments, we observe that the distillation process is able to improve the performance of the student model when trained over thousands of labeled instances per class. In this setting, we consider only $500$ labeled samples per class for every task, while the remaining instances are considered as unlabeled in our framework. The objective of this experiment is to find out scenarios where distillation with unlabeled data provides maximum value. Table~\ref{tab:less} summarizes the results.

\begin{table}[]
    \centering
    \begin{tabular}{lcccc}
\toprule
{ Dataset} & { RNN} & { Student} & { Student}  &	{ BERT}\\
 &  & { no distil.} & { with distil.}  &	{ Large}\\
\midrule
AG News & 85.03 &	85.85 &	{\bf 90.45} &	90.36\\
IMDB & 52.94 &	61.53 &	89.08 &	{\bf 89.11}\\
Elec & 68.93 &	65.68	& {\bf 91.00}	& 90.41\\
DBpedia & 93.33 &	96.30 &	{\bf 98.94}	& {\bf 98.94}\\
\bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Distillation with BERT Large on $500$ labeled samples per class.}
    %\vspace{-1.5em}
    \label{tab:less}
\end{table}

We observe a huge improvement in performance on distilling the student model from BERT Large when there are limited number of labeled samples per class. The distilled student improves over the non-distilled version by $19.4$ percent and matches the teacher performance for all of the tasks.

\begin{table}[]
%\vspace{-1em}
    \centering
    \begin{tabular}{lccc}
    \toprule
    Dataset & Student & Student & BERT \\
    & Hard Distil. & Soft Distil. & Large \\\midrule
    IMDB &  87.37 & {\bf 87.84} & 87.72\\
    Elec  & 89.17 & {\bf 90.14} & 89.94\\
        \bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Distillation with BERT Large (with pre-training and fine-tuning) on $100$ labeled samples per class.}
    %\vspace{-0.5em}
    \label{tab:small}
\end{table}

\subsubsection{$100$ labeled samples per class} In this setting, we consider only $100$ labeled samples per class for training all models. When we fine-tuned BERT Large on this small labeled set, the accuracy was similar to the previous case ($500$ labeled samples per class) for DbPedia and AG News dataset. However, for IMDB and Elec datasets BERT accuracy was $50\%$ (random) for binary classification. Therefore, we now turn our focus to these two challenging datasets for this setting.

First, we pre-train the BERT Large language model on these two datasets starting from the checkpoints. Second, we fine-tune the model for classification tasks. Note that for all of the previous experiments, we only performed the second step and never pre-trained the language models. Surprisingly, its performance now improved drastically. Next, we distil the student model from the fine-tuned BERT Large classifiers. Table~\ref{tab:small} summarizes the results. We observe that the student model now exceeds the BERT Large performance with just $100$ labeled samples per class. In contrast to the previous settings where we did not perform the language model pre-training, the student model is now able to exploit the soft representations better from the teacher.

%Overall, we observe that the distilled student model matches or outperforms the teacher in case of small labeled training sets. This is because the distillation framework exploits the teacher uncertainties and provides better regularization which is all the more required in this setup.

\subsection{Impact of Training Schedule on Distillation}

We had proposed three different schedules for distilling the student model based on joint and stagewise optimization with gradual unfreezing. From Table~\ref{tab:training} we observe that the different training schedules does impact the distillation performance. We observe that the stagewise schedule ({\small $\mathcal{R_{RL}}\ | \mathcal{R_{LL}} + \mathcal{R_{CE}}$} in table) where we first optimize the loss $\mathcal{R_{RL}}$ (cf. Equations~\ref{eq:5},~\ref{eq:6}) between the representations of the student and teacher model from the final layer, and then jointly optimize for the cross-entropy loss $\mathcal{R_{CE}}$ (cf. Equations~\ref{eq:1},~\ref{eq:2}) and logit loss $\mathcal{R_{LL}}$ (cf. Equations~\ref{eq:3},~\ref{eq:4}) with gradual unfreezing performs the best.

\begin{table}[]
    \centering
    \begin{tabular}{lccc}
\toprule
Dataset & {\small $\mathcal{R_{RL}}\ |$} & {\small $\mathcal{R_{RL}} +$} &
{\small $\mathcal{R_{RL}}+ \mathcal{R_{LL}}\ |$}\\
 & {\small $\mathcal{R_{LL}} + \mathcal{R_{CE}}$} & {\small $\mathcal{R_{LL}} + \mathcal{R_{CE}}$} &
{\small $\mathcal{R_{CE}}$}\\
\midrule
Ag News	& {\bf 92.33} &	92.17 &	92.26\\
IMDB & {\bf 91.22} &	90.07 & 90.87\\
Elec & {\bf 93.55} &	{93.12} & 93.10\\
DbPedia	 & {\bf 99.10} & {99.08} & {99.08}\\
\midrule
Ag News	& {\bf 94.33} &	93.90 &	93.78\\
IMDB & {\bf 91.70} &	90.84 & 90.89\\
Elec & {\bf 93.56} &	93.16 & 93.35\\
DbPedia	 & {\bf 99.06} & {99.06} & 99.04 \\
\bottomrule
    \end{tabular}
    %\vspace{-0.5em}
    \caption{Different training schedules for distillation with BERT. `$|$' indicates different stages and `$+$' indicates joint optimization. The first block shows distillation results with BERT Base and the second block with BERT Large. The training scheme in the first column optimizes the representation loss in the first stage, and then jointly optimizes the logit loss and cross-entropy loss in the second stage with gradual unfreezing of the layers. The one in the second column optimizes all the loss functions jointly. Whereas the last one first optimizes the representation and logit loss over unlabeled data, followed by fine-tuning on labeled data.}
    %\vspace{-1em}
    \label{tab:training}
\end{table}

\subsection{Summary of Findings}
In this work, we make the following observations:

\noindent $\bullet$  RNN encoders (with word embeddings) work very well for distilling large pre-trained language models. We also experimented with encoders like deep multi-layer CNN as in~\citep{DBLP:journals/corr/RomeroBKCGB14,DBLP:conf/nips/ZhangZL15}. However RNNs performed much better.

\noindent $\bullet$  Several architectural choices like width of the student network, sequence length, regularization (e.g., dropouts) and optimization algorithm impact distillation performance.

\noindent $\bullet$  Students with distillation greatly outperform those without in settings with limited amount of labeled data, large amount of in-domain unlabeled data, and a good teacher.

\noindent $\bullet$  Large pre-trained language models make very confident predictions. This makes soft distillation difficult which is more effective in presence of teacher uncertainties and possibly a large label space.

\noindent $\bullet$  Increasing the size of the teacher leads to marginal gain in the distillation process without increasing the size of the student network once it saturates.

\noindent $\bullet$  Training schedule for optimizing multiple loss functions impact distillation where stagewise training with gradual unfreezing works best.

\begin{comment}
\subsection{Distil Once Fine-tune Forever}
In this experiment, we want to find if the distilled student model further improves in performance as we have more labeled data available over time. To this end, we first train the student model over data in Table~\ref{XXX}. Recall that for AG News and Dbpedia we used only a fraction of the data for distilling while treating the remaining as unlabeled. Now during the second phase, we can continue training the distilled model to optimize for the cross-entropy loss over the fully available labeled data as in Table~\ref{XXX}. The results are summarized in Table~\ref{XXX}. 

\begin{table}[]
    \centering
    \begin{tabular}{lcc}
    Dataset & Distil Phase & Fine-tune Phase &
    \midrule
    AG News & 92.33 & 93.53\\
    DBpedia & 99.08 & 99.12\\
    \midrule
    AG News & 94.33 & 94.41\\
    Dbpedia & &\\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
\end{comment}


